SCALE-Sim: Systolic CNN Accelerator Simulator

Systolic Arrays are one of the most popular compute substrates within Deep Learning accelerators today, as they provide extremely high efficiency for running dense matrix multiplications. However, the research community lacks tools to insights on both the design trade-offs and efficient mapping strategies for systolic-array based accelerators. We introduce Systolic CNN Accelerator Simulator (SCALE-Sim), which is a configurable systolic array based cycle accurate DNN accelerator simulator. SCALE-Sim exposes various micro-architectural features as well as system integration parameters to the designer to enable comprehensive design space exploration. This is the first systolic-array simulator tuned for running DNNs to the best of our knowledge. Using SCALE-Sim, we conduct a suite of case studies and demonstrate the effect of bandwidth, data flow and aspect ratio on the overall runtime and energy of Deep Learning kernels across vision, speech, text, and games. We believe that these insights will be highly beneficial to architects and ML practitioners.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The case study covers the insights that we want to convey. However, there could be other high level intuitions and qualitative insights that we might choose not to discuss in details. 

This section is a placeholder for them. Once the paper takes shape we can decide weather to keep this or not.


==> packages_2.tex <==
\usepackage{amsmath}
\usepackage{algorithmic}
\usepackage[linesnumbered]{algorithm2e}
\usepackage{color}

%\usepackage[hyphens]{url}
%\usepackage{breakurl}
%\usepackage[breaklinks,colorlinks,bookmarks=false]{hyperref}
%\usepackage{hyperref}

\usepackage[usenames,dvipsnames]{xcolor}
%\hypersetup{citecolor=blue,linkcolor=blue}


\usepackage{graphicx}
\usepackage{listings}
\usepackage{setspace}
\usepackage{caption}
\usepackage{comment}
\usepackage{floatrow}
\usepackage{subfigure}
\usepackage[most]{tcolorbox}

\usepackage{endnotes,microtype,xspace,graphicx,fancyvrb,multirow}
\usepackage{fancyhdr}
\usepackage[normalem]{ulem}
\usepackage[hyphens]{url}


==> packages_orig.tex <==
\usepackage{amsmath}
\usepackage{algorithmic}
\usepackage[linesnumbered]{algorithm2e}
\usepackage{color}
\usepackage{footnote}

%\usepackage{hyperref}

\usepackage{graphicx}
\usepackage{listings}
%\usepackage{setspace}
\usepackage{caption}
\usepackage{comment}
\usepackage{hyperref}
%\usepackage[most]{tcolorbox}
%
%\usepackage{endnotes,microtype,xspace,graphicx,fancyvrb,multirow}
%\usepackage{fancyhdr}
%\usepackage[normalem]{ulem}
%\usepackage[hyphens]{url}
%\usepackage[bookmarks=true,breaklinks=true,letterpaper=true,colorlinks,linkcolor=black,citecolor=blue,urlcolor=black]{hyperref}


